Guarding a Translating Line with an Attached Defender

In this paper we consider a Target-guarding differential game where the Defender must protect a linearly moving line segment by intercepting the Attacker who tries to reach it. In contrast to common Target-guarding problems, we assume that the Defender is attached to the Target and moves along with it. This assumption affects the Defender's maximum speed depending on its heading direction. A zero-sum differential game of degree for the Attacker-winning scenario is studied, where the payoff is defined to be the distance between the two agents at the time of reaching the Target. We derive the equilibrium strategies and the Value function by leveraging the solution for the infinite-length Target scenario. The zero-level set of this Value function provides the barrier surface that divides the state space into Defender-winning and Attacker-winning regions. We present simulation results at the end to demonstrate the theoretical results.

==> infinite_length_target_daigo.tex <==
As a building block towards the complete solution, we first assume the length of the Target to be infinite. The speed of the target still affects the game through the relative speed that the Defender can achieve.

For this alternate version of the problem, the Attacker can win the game by reaching the following terminal surface $\mathcal{S_T}$, which is $x$-axis of the moving frame:
\begin{align}\label{terminal_cond_inf}
    \mathcal{S_T} = \{\hat{\textbf{x}} \hspace{1mm} \mid \hspace{1mm} \hat{y}_A(t_f) = 0\}.
\end{align}
%where, $R = |x_A - x_D|$.
Assumptions 1 and 2 are retained for this analysis.

\subsection{First Order Necessary Conditions for Optimality} 
The kinematics remain unchanged from the previous analysis;
The Hamiltonian for the differential game is defined as,
\begin{equation}\label{hamiltonian}
    \begin{aligned}
    \mathcal{H}_d &=  
    \sigma_{\hat{x}_D} w_D + 
    \sigma_{\hat{x}_A} v_A\cos{\phi_A} - \sigma_{\hat{x}_A} v_T + \sigma_{\hat{y}_A} v_A\sin{\phi_A} ,
\end{aligned}
\end{equation}
where, $\sigma \equiv [\sigma_{\hat{x}_D} \hspace{3mm} \sigma_{\hat{x}_A} \hspace{3mm} \sigma_{\hat{y}_A}]^T$ is the adjoint vector.
The Hamiltonian is a separable function
of the controls $w_D$ and $\phi_A$, and thus \textit{Isaacs’ condition} \cite{Issacs1965} , \cite{Basar2011} holds:
\begin{align}
    \min\limits_{w_D(t)} \max\limits_{\phi_A(t)} \mathcal{H} = \max\limits_{\phi_A(t)} \min\limits_{w_D(t)} \mathcal{H}.
\end{align}
The equilibrium adjoint dynamics are given by,
% \begin{subequations}\label{adjoint_def}
    \begin{align}
    \dot{\sigma}_{\hat{x}_D} &= \frac{\partial \mathcal{H}}{\partial \hat{x}_D} = 0\\
    \dot{\sigma}_{\hat{x}_A} &= \frac{\partial \mathcal{H}}{\partial \hat{x}_A} = 0\\
    \dot{\sigma}_{\hat{y}_A} &= \frac{\partial \mathcal{H}}{\partial \hat{y}_A}
    = 0
\end{align}
% \end{subequations}

The terminal adjoint values are obtained from the transversality condition \cite{Bryson1975}
%In optimal control theory, a transversality condition is a boundary condition for the terminal values of the costate variables. They are one of the necessary conditions for optimality in finite-horizon optimal control problems without an endpoint constraint on the state variables
\begin{equation}
    \begin{aligned}
    \sigma^T(t_f) &= 
    \begin{bmatrix}
    \sigma_{\hat{x}_D}(t_f) & \sigma_{\hat{x}_A}(t_f) & \sigma_{\hat{y}_A}(t_f)
    \end{bmatrix}
    \\
    &=\frac{\partial \Phi}{\partial \hat{\textbf{x}}_f} + \eta \frac{\partial \phi}{\partial \hat{\textbf{x}}_f}   \\
            &= \begin{bmatrix}
              \frac{\hat{x}_D- \hat{x}_A}{|\hat{x}_A - \hat{x}_D|} & \frac{\hat{x}_A - \hat{x}_D}{|\hat{x}_A - \hat{x}_D|} & 0
              \end{bmatrix} +
              \eta
              \begin{bmatrix}
              0 & 0 & 1
              \end{bmatrix}
    \\
    &=  \begin{bmatrix}
    \lambda & -\lambda & \eta
    \end{bmatrix},
    \\
\text{ where, } \lambda &= \text{sign}(\hat{x}_A - \hat{x}_D).
\end{aligned}
\end{equation}

Therefore, with (16)-(19), the following hold,
\begin{equation}
    \begin{aligned}
    \sigma_{\hat{x}_D}(t) &= \lambda,   &\forall \hspace{0.0mm} t \in [t_0, t_f]\\
    \sigma_{\hat{x}_A}(t) &= -\lambda,    &\forall \hspace{0.0mm} t \in [t_0, t_f]\\
    \sigma_{\hat{y}_A}(t) &= \eta, &\forall \hspace{0.0mm} t \in [t_0, t_f].
\end{aligned}
\end{equation}
The terminal Hamiltonian satisfies,
\begin{equation}
     \begin{aligned}
     \mathcal{H}(t_f) = -\frac{\partial \Phi}{\partial t_f} -\eta \frac{\partial\phi}{\partial t_f} &= 0
 \end{aligned}
\end{equation}
and $\frac{d\mathcal{H}}{dt} = 0$, so, $\mathcal{H}(t) = 0$ for all $t \in [t_0, t_f]$.


The equilibrium control actions of the Attacker and Defender maximize and minimize (\ref{hamiltonian}) respectively: $\mathcal{H}^* = \text{max}_{\phi_A} \text{min}_{w_D} \mathcal{H}$. 
For the saddle point solution of the problem, we have
\begin{equation}\label{wd*}
    \begin{aligned}
    w_D^* &= \argminD_{w_D} \mathcal{H}
    \\ &= \argminD_{w_D} (\sigma_{\hat{x}_D}w_D) = -\text{sign}({\sigma_{\hat{x}_D}}) = -\lambda
    \end{aligned}
\end{equation}
\begin{equation}\label{phi*}
    \begin{aligned}
    \phi_A^* &= \argmaxD_{\phi_A} \mathcal{H}\\
    &= \argmaxD_{\phi_A} (\sigma_{\hat{x}_A} v_A\cos{\phi_A} + \sigma_{\hat{y}_A} v_A\sin{\phi_A})
    \end{aligned}
\end{equation}
Solving (\ref{phi*}) we have
\begin{equation}\label{cosphi*}
    \begin{aligned}
    \cos{\phi_A}^* &= \frac{\sigma_{\hat{x}_A}}{\sqrt{\sigma_{\hat{x}_A}^2 + \sigma_{\hat{y}_A}^2}}  = \frac{-\lambda}{\sqrt{\eta^2 + 1}}.
    \end{aligned}
\end{equation}
\begin{equation}\label{sinphi*}
    \begin{aligned}
    \sin{\phi_A}^* &= \frac{\sigma_{\hat{y}_A}}{\sqrt{\sigma_{\hat{x}_A}^2 + \sigma_{\hat{y}_A}^2}} = \frac{\eta}{\sqrt{\eta^2 + 1}}
    \end{aligned}
\end{equation}
 
If $\eta < 0$, this implies $\sin{\phi_A^*}<0$ due to (\ref{sinphi*}). However, this would mean $\phi_A \in [-\pi, 0]$. Thus, it must be the case that $\eta > 0$.


Substituting the equilibrium controls, (\ref{wd*}), (\ref{cosphi*}) and (\ref{sinphi*}), into the Hamiltonian, (\ref{hamiltonian}), and evaluating at terminal time with adjoints gives
\begin{equation}
\begin{aligned}
    \mathcal{H}^*(t_f) = 0 =
    & \lambda(-\lambda) + (-\lambda)v_A\bigg(\frac{-\lambda}{\sqrt{\eta^2 + 1}}\bigg)  \\  &- (-\lambda) v_T + \eta  v_A\bigg(\frac{\eta}{\sqrt{\eta^2 + 1}}\bigg)
    \\
    \Longrightarrow \eta  =& \pm\frac{\sqrt{(1 - \lambda v_T)^2 - v_A^2}}{v_A}.
\end{aligned}
\end{equation}
Since $\eta > 0$, we have
\begin{equation}
    \begin{aligned}
    \eta  &= \frac{\sqrt{(1 - \lambda v_T)^2 - v_A^2}}{v_A}
    \end{aligned}
\end{equation}


%=====================================%
\subsection{Solution Characteristics}
The retrograde equilibrium kinematics can be obtained by substituting the equilibrium controls, (\ref{wd*}), (\ref{cosphi*}) and (\ref{sinphi*}), along with the adjoints into (\ref{Attacker_dyn_mf}) which yields
\begin{equation}\label{xA_dot}
\begin{aligned}
\dot{\hat{x}}_A &= -v_T - \frac{\lambda v_A^2}{1-\lambda v_T}
\end{aligned}
\end{equation}

\begin{equation}\label{yA_dot}
\begin{aligned}
\dot{\hat{y}}_A &= v_A \sqrt{1-\bigg(\frac{v_A}{1-\lambda v_T}\bigg)^2} 
\end{aligned}
\end{equation}
with boundary conditions,
\begin{align}
    \hat{y}_A(t_f)=0 , \quad |\hat{x}_A(t_f)-\hat{x}_D(t_f)| > 0.
    %have to consider where less than l
\end{align}


Now, considering the relative position $x=\hat{x}_A-\hat{x}_D$ and $y=\hat{y}_A-\hat{y}_D=\hat{y}_A$, we have
\begin{equation}\label{m1}
    \begin{aligned}
            \frac{dy}{dx} = m_1 \triangleq \frac{v_A\sqrt{\rho^2 -v_A^2}}{\rho(\lambda-v_T)-\lambda v_A^2}, 
            % \\
            % \Longrightarrow y &= m_1 x + C; \\
            % & \text{where, } m_1 =\frac{v_A\sqrt{\rho^2 -v_A^2}}{\rho(\lambda-v_T)-\lambda v_A^2} \in {\RR}
    \end{aligned}
\end{equation}
where $\rho := 1- \lambda v_T$.
This implies that the equilibrium trajectories of the system in the $xy$-plane is given by straight lines:
\begin{equation}
    y = m_1 x + C.
\end{equation}
Note that, the value of $m_1$ depends on $\lambda\equiv\text{sign}(x)$.
Figure~\ref{fig:flow_field} presents the equilibrium trajectories for initial conditions satisfying $y(0)<0$.
Recalling that $x=0$ (y-axis) is part of the terminal surface corresponding to Defender's win, and $y=0$ (x-axis) is the one corresponding to Attacker's win, every trajectory terminates when it hits either of the two axes.

\begin{figure}[h!]
    \centering
    \includegraphics[width = 9.5 cm]{images/combined.png}
    \caption{Full Equilibrium Flow Field with $v_A = 0.7$ and $v_T = 0.2$}
    \label{fig:flow_field}
\end{figure}

% In equation (\ref{m1}), if $C = 0$, $m_1$ represents the Barrier surface defined by equation (10) and shown in figure (\ref{fig:flow_field}).

% In figure (\ref{fig:flow_field}), for the given values of the Attacker and Target speed, we can see the Attacker winning Region, $\mathcal{R}_A$ and the Defender winning region $\mathcal{R}_D$ separated by the Barrier surface shown as the Black lines. The value of the game is constant for a given set of Defender and Attacker position. The value of the game can be obtained by following the Line from initial position of the Attacker to Terminal Surface: horizontal thick Red line when the Attacker is winning and vertical thick blue line when the Defender is winning.


\subsection*{Domain of the Attacker Speed:} Considering the differential equation obtained by dividing the equation (\ref{yA_dot}) and (\ref{xA_dot})
\begin{align*}
    & \frac{dy_A}{dx_A} = m_2 \triangleq \frac{v_A\sqrt{\rho^2 -v_A^2}}{-v_T (\rho -\lambda)},
\end{align*}
which implies that the Attacker's trajectory in the moving frame can be described as
\begin{equation}
   y_A =  m_2 x_A + C.
\end{equation}
% \textit{Case 1:} 

When Defender is ahead of the Attacker i.e. $x_D>x_A$, $\lambda = +1$, from equation (29) we get,
\begin{align}
    m_2 &= \frac{v_A}{-v_T^2} \sqrt{(1-v_T)^2 - v_A^2}.
\end{align} 
For this slope to be a real number, we need $(1-v_T)^2 - v_A^2 \geq 0$, which is equivalent to
\begin{align}
    0 < v_A < 1-v_T.
\end{align}
If Attacker's maximum speed violates this condition (i.e., $v_A>1-v_T$), it implies that Attacker can move faster than the Defender in the negative $x$ direction.
Consequently, it can always reach the infinite length Target without being intercepted by the Defender.

% which implies in this scenario, the Defender speed, $w_D = 1-v_T$. 
% If the Attacker moves faster than $w_D$ it will violate the assumption $1$ and consequently, it can always reach the infinite length Target without being intercepted by the Defender.
% \textit{Case 2:} 
When the Defender is ahead of the Attacker i.e. $x_D<x_A$, $\lambda = -1$, the slope of the Attacker's optimal trajectory in the moving frame is 
\begin{align}
    m_2 = \frac{v_A\sqrt{(1+v_T)^2 -v_A^2}}{-v_T (2+ v_T)}.
\end{align}
% \begin{align}
%     (v_T + 1)^2 - v_A^2 \geq 0
%     \quad &\Longrightarrow 0 < v_A < 1+v_T,
% \end{align}
% which suggests the same conclusion as assumption $1$.
The slope $m_2$ is always real value under Assumption 1.

\begin{theorem}[Solution for Infinite-Length Target]
When the Target is infinite and moving at a constant velocity, the equilibrium state feedback control strategies for the \textit{Game of Degree} are, 
\\
if the Attacker is ahead of the Defender:
\begin{equation}
\begin{aligned}
\cos{\phi_A}^* &= \frac{-v_A}{1-v_T}
                \\ 
\sin{\phi_A}^* &= \frac{\sqrt{(1-v_T)^2-v_A^2}}{1-v_T}
                \\
w_D^* &= 1,
\end{aligned}
\end{equation}
and conversely, if the Defender is ahead of the Attacker:
\begin{equation}
\begin{aligned}
\cos{\phi_A}^* &= \frac{v_A}{1+v_T}
\\ 
\sin{\phi_A}^* &= \frac{\sqrt{(1+v_T)^2-v_A^2}}{1+v_T}
\\
w_D^* &= -1.
\end{aligned}
\end{equation}
The Value of the Game is,
\begin{equation}
    \begin{aligned}\label{Value}
     V &= \hat{x}_A(t)-  \hat{x}_D(t) -\frac{\hat{y}_A}{v_A\sin{\phi_A^*}}(v_A \cos{\phi_A^*-w_D^*-v_T}).
\end{aligned}
\end{equation}

\end{theorem}

\begin{proof}
We can check following the infinite-length Attacker-strategy at which point Attacker will intercept the Target, if there is no intervention. Then we consider the time to reach that point for both the Defender and the Attacker from their initial position to determine if the Defender can intercept the Attacker before reaching the Target.
\\
The speed of the Attacker in moving frame while pursuing the Target,
\begin{align}\label{rel_speed_A}
    \hat{v}_A &= \sqrt{(v_A \cos{\phi_A^*-v_T})^2+(v_A\sin{\phi_A^*})^2}.
\end{align}

Attacker's heading angle in moving frame,
\begin{align}\label{inf_theta}
    \cos{\hat{\phi}}_A &= \frac{v_A\cos{\phi}_A^*-v_T}{\hat{v}_A} 
    \\
    \sin{\hat{\phi}}_A &= \frac{v_A\sin{\phi}_A^*}{\hat{v}_A}
\end{align}

Now, let's assume if the Attacker follows the infinite length strategy (\ref{inf_theta}) along with the speed $\hat{v}_A$, it is can reach the infinitely long Target. If the Attacker starts from a point $A(\hat{x}_A,\hat{y}_A)$ and reaches the Target at any point $B(\hat{x}_B,\hat{y}_B)$, we can compute,

\begin{align}\label{x_B}
    \hat{y}_A-\hat{y}_B &= (\hat{x}_A-\hat{x}_B)\tan{\hat{\phi}_A} 
    \\
    \hat{x}_B &= \hat{x}_A - \frac{\hat{y}_A\cos{\hat{\phi}_A}}{\sin{\hat{\phi}_A}}
\end{align}
If It takes time, $t_A$ to reach $B$ for the Attacker and $t_D$ for the Defender:
\begin{align}
    t_D &= \bigg|\frac{\hat{x}_D-\hat{x}_B}{w_D}\bigg|
    \\
    t_A &= \frac{\sqrt{(\hat{x}_B-\hat{x}_A)^2+(\hat{y}_B-\hat{y}_A)^2}}{\hat{v}_A}.
\end{align}
If $t_D > t_A$: the Attacker takes less time than the Defender to reach $B$, thus \text{Attacker Wins} in this case; the terminal time $t_f$ will be the time consumed by the Attacker to reach Target
\begin{align}
    t_f = t_A.
\end{align}
Defenders position at terminal time is 
\begin{align}
    \hat{x}_D(t_f) &= \hat{x}_D(t)+w_D t_f.
\end{align}
At terminal time $\hat{x}_A$ will approach $\hat{x}_B$ as derived in equation (\ref{x_B}), and $\hat{x}_D(t)$ will approach $\hat{x}_D(t_f)$.
\end{proof}

